Tradeoffs for small-depth Frege proofs

We study the complexity of small-depth Frege proofs and give the first tradeoffs between the size of each line and the number of lines. Existing lower bounds apply to the overall proof size -- the sum of sizes of all lines -- and do not distinguish between these notions of complexity. For depth-$d$ Frege proofs of the Tseitin principle on the $n \times n$ grid where each line is a size-$s$ formula, we prove that $\exp(n/2^{\Omega(d\sqrt{\log s})})$ many lines are necessary. This yields new lower bounds on line complexity that are not implied by H{\aa}stad's recent $\exp(n^{\Omega(1/d)})$ lower bound on the overall proof size. For $s = \mathrm{poly}(n)$, for example, our lower bound remains $\exp(n^{1-o(1)})$ for all $d = o(\sqrt{\log n})$, whereas H{\aa}stad's lower bound is $\exp(n^{o(1)})$ once $d = \omega_n(1)$. Our main conceptual contribution is the simple observation that techniques for establishing correlation bounds in circuit complexity can be leveraged to establish such tradeoffs in proof complexity.

==> old-obtain.tex <==

Let $\calP$ be a depth-$d$
refutation of $\Tseitin({\exG}_n[\alpha])$ where $d \leq d^\star =  c \sqrt{\log n}$,
and let $\calP^*$ be the multiset of all subformulas of $\calP$.
The main result of this section (Lemma~\ref{lemma:restriction-evaluation}) 
uses our final switching lemma (Theorem~\ref{thm:final-SL-stringy}, stated below) to prove that 
if $\calP$ is ``small'', then there exists a pair $(\rho^{(d)},H^{(d)})  \in \supp({\cal A}^{(d)})$ such that 
the multiset, $\calP^* \uhr \rho^{(d)}$ will have a $k$-evaluation
where $k = (\log n)/200d$.  
Recall that $\calP \uhr \rho^{(d)}$ is a depth-$d$ refutation of
$\Tseitin(H^{(d)}[\alpha^{(d)}])$ where $\alpha^{(d)} = \alpha \uhr \rho^{(d)}$, and observe that $\calP^* \uhr \rho^{(d)}$ is the multiset of all occurrences of subformulas in $\calP \uhr \rho^{(d)}$. 
Applying Lemma \ref{lemma:k-eval-frege} (with its $P$ being $\calP \uhr \rho^{(d)}$ and its $P^*$ being $\calP^* \uhr \rho^{(d)}$), it follows that 
$\calP \uhr \rho^{(d)}$ cannot be a refutation of $\Tseitin(H^{(d)}[\alpha^{(d)}])$,
which contradicts our assumption that $\calP$ is a ``small'' refutation
of $\Tseitin({\exG}_n[\alpha])$.


\begin{lemma}[Lemma 7.1 in \cite{PRST}]
\label{lemma:restriction-evaluation}
Let $\calP$ be a size $(s,S)$ depth-$d$ Frege proof of $\Tseitin({\exG}_n[\alpha])$, 
where $d \leq d^\star$. 
If $s < bla$ and $S < bla$, then there exists a pair 
$(\rho^{(d)},H^{(d)}) \in \supp({\cal A}^{(d)})$ such that
$\calP \uhr {\rho}^{(d)}$ has a $k$-evaluation where
$k = td+l$, $t = bla$ and $l = bla$.
\end{lemma}


As discussed above, 
Theorem \ref{thm:main} follows directly from Lemmas~\ref{lemma:k-eval-frege} and Lemma~\ref{lemma:restriction-evaluation}, 
observing that $(\log n)/200d \ll \tau(d,n)/(3\lambda^\star)$. 

We now state our final switching lemma.  
The rest of this paper after Section \ref{sec:obtaining-k-eval}
is devoted to proving Theorem \ref{thm:final-SL-stringy}. 

\begin{theorem} [Final switching lemma] \label{thm:final-SL-stringy} 
NEED TO RESTATE THIS. Let $0 \leq i \leq d < d^\star.$
Fix $(\rho^{(i)},H^{(i)}) \in \supp(\calA^{(i)})$. Let $T_1,\dots,T_M$ be $(k,H^{(i)})$-good decision trees over $E(H^{(i)})$ \red{where $k = (\log n)/200d$} and let $\alpha' = \alpha \uhr \rho^{(i)}$.
Then except with failure probability at most \red{$n^{-\eps(\log n)/d^2}$} over a 
draw of $(\brho^{(i+1)},\bH^{(i+1)}) \sim \calA^{(i+1)}(\rho^{(i)},H^{(i)})$,
 there is a $(\red{k}, \bH^{(i+1)})$-good decision tree over $E(\bH^{(i+1)})$ that $(\bH^{(i+1)}, \alpha' \uhr \brho^{(i+1)})$-represents $\lor_j \Prune_{\bH^{(i+1)}, \alpha'\uhr\brho^{(i+1)}}(T_j\uhr \brho^{(i+1)})$.
\end{theorem}


\noindent{\bf High Level Overview.} Using the switching lemma, we will prove by induction on $i$, $i \leq d$, that there exists a restriction
$\rho^{(i)}$ and a mapping $\calT^i$ which assigns to each
occurrence of a subformula in the proof $P$ a decision tree of height
at most $ti +l $ satisfying the properties in the definition of
a $k$-evaluation.

To do this we will define the following process which iteratively applies
a good restriction in order to reduce the depth of each formula in the proof.
Initially when $i=0$, we start with the multiset of depth at most $d$ formulas.
For $i=1$, using the switching lemma, we argue that there
exists a good restriction $\rho_1$ such that for each formula $F$ in the proof,
all depth-1 subformulas of $F$ have a common canonical
decision tree.
We repeat this for $d$ stages, using good restrictions $\rho_1,\ldots,\rho_d$.
At each stage $i \leq d$, we grow the common decision tree associated with
all subformulas of $F$, increase the common tree from depth $t(i-1)$ to depth $ti$
by adding $t$ new layers to the common tree.



\subsection{Proof of Lemma~\ref{lemma:restriction-evaluation}

\begin{proof}(Proof of Lemma~\ref{lemma:restriction-evaluation})
Let $P$ be our original size $(s,S)$ depth-$d$ refutation of $\Tseitin({\exG}_n[\alpha])$
and let $P^*$ be the multiset of all subformulas of $P$
(where subformulas are with respect to unbounded-fanin).
Given $i \in [d]$, and a formula $F \in P$, let
$F_{\leq i}$ denote the set of all subformulas of $F$
of depth at most $i$, and let $F_i$ denote the set of all subformulas of $F$ of depth exactly $i$.
$F_i$ is the disjoint union of $F_{\lor,i}$ and $F_{\neg,i}$ where
$F_{\lor,i}$ are the depth $i$ subformulas of $F$ where the top gate
is an unbounded fanin OR gate, and $F_{\neg,i}$ are the depth-$i$
subformulas of $F$ where the top gate is negation.
Finally, let $\Gamma_i$ be the multiset consisting of $\cup_{F \in P} F_i$,
and let $\Gamma_{\leq i}$ be the multiset of formulas $\cup_{F \in P} F_{\leq i}$.
Again, $\Gamma_i$ is the disjoint union of $\Gamma_{\lor,i}$ and $\Gamma_{\neg,i}$.

We will first prove by induction on $i$,
that there exists a pair $(\rho^{(i)},H^{(i)}) \in \supp({\cal A}^{(i)})$
and a mapping $\calT^{(i)}$ such that the following holds:
for every formula $F \in P$ there exists a {\it common} 
tree $T^{F,i}$ of depth $ti$ such that for every
$A^F \in F_{\leq i}$,
$\calT^{(i)}(A^F \uhr \rho^{(i)})$ will be mapped to a $(ti+l,H^{(i)})$-good
decision tree where the common tree $T^{F,i}$ is at the top,
followed by $l$ layers at the bottom that are specific to $A^F \uhr \rho^{(i)}$.
After defining our mapping $\calT^{(i)}$, we will then prove inductively that it
satisfies the properties of a $k$-evaluation (Definition \ref{def:keval}).

For the base case when $i=0$, recall that
${\cal A}^{(0)}$ is the empty restriction.
For $b \in \{0,1\}$, we define $\calT^{(0)}(b)=b$ ( the one-node tree comprising a single leaf labelled by $b$).
If $e$ is a variable, then we define
$\calT^{(0)}(e)$ to be the depth-1 tree that queries this variable,
where the path $e=0$ has leaf value $0$ and the path $e=1$ has
leaf value $1$.
Similarly we define $\calT^{(0)}(\neg e)$ to be the depth-1
tree where $e$ is queried and the path $e=0$ has leaf value $1$
and the path $e=1$ has leaf value $0$.
It is easy to check that these trees are $(k,G_n)$-good and
satisfy the properties of Definition \ref{def:keval}.


Now assume by the inductive hypothesis that there
exists a pair $(\rho^{(i)},H^{(i)})\in \supp(H^{(i)})$ and a mapping $\calT^{(i)}$ satisfying
the properties described above.
Note that $\Gamma_{\leq i+1}$ is the disjoint union of the multisets 
$\Gamma_{\lor,i+1}$, $\Gamma_{\neg,i+1}$, and $\Gamma_i$.

\begin{itemize}
\item[(a)] First consider formulas $A \in \Gamma_{\lor,i+1}$.
Each such $A$ is a subformula of some $F \in P$, so we will write this
occurrence of $A$ as $A^F$ to indicate that it is a copy of $A$ occurring in $F$.
Since $A^F \in \Gamma_{\lor,i+1}$, $A^F$ is the disjunction of some set of
at most $s$ formulas, $A_1^F,\ldots,A_s^F \in F_{\leq i}$.
By the induction hypothesis, for all such $A_j^F$ the tree
$\calT^{(i)}(A_j^F \uhr \rho^{(i)})$ is a
$(ti+l,H^{(i)})$-good decision tree satisfying properties (1)-(3) of Definition~\ref{def:keval}.
In particular, $\calT^{(i)}(A_j \uhr \rho^{(i)})$ consists of
the common tree $T^{F,i}$ of height $ti$ at the top, 
and for each branch $\sigma \in \Branches(T^{F,i})$, the leaf associated with $\sigma$ in $T^{F,i}$ is
labelled with a height-$l$ subtree, $\calT^{(i)}(A_j^F \uhr \rho^{(i)}) \uhr \sigma$ (specific to $A_j^F$).


For a pair $(F,\sigma)$, where $F \in P$, and $\sigma \in \Branches(T^{F,i})$, 
we define ${\cal S}(F,\sigma)$ to be the following
set of $l$-DNF formulas:
$${\cal S}(F,\sigma) = \{ \lor_{j=1}^s Disj( \calT^{(i)}(A_j^F \uhr \rho^{(i)})) \uhr \sigma ~:~ A^F = A_1^F \lor \ldots A_s^F, ~ A^F \in F_{\lor,i+1} \} .$$

We want show that under a suitable restriction 
every set of $l$-DNF formulas
${\cal S}(F,\sigma)$, $F \in P$, $\sigma \in T^{F,i}$, has a common canonical $(t,l)$ decision tree.
That is, for each ${\cal S}(F,\sigma)$, there exists a {\it common} tree $T(F,\sigma)$ of height $t$
such that each $l$-DNF formula in ${\cal S}(F,\sigma)$ can be written as a height $t+l$ decision tree,
where $T(F,\sigma)$ is at the top, followed by height-$l$ trees as the leaves.

The existence of such a good restriction follows from
our main multiswitching lemma: For each pair $(F,\sigma)$, $|{\cal S}(F,\sigma)| \leq s$,
and the number of sets ${\cal S}(F,\sigma)$ is at most $S \cdot 2^{ti}$ and thus applying
Theorem~\ref{thm:final-SL-stringy} together with a union bound (over $S 2^{ti}$ sets),
we get that there exists some
$(\rho^{(i+1)},H^{(i+1)}) \in \supp(\calA^{(i+1)}(\rho^{(i)},H^{(i)}))$ satisfying the following:
for all $F \in P$, and for all $\sigma \in \Branches(T^{F,i})$, there is a $(t,l)$-CCDT,
for all sets ${\cal S}(F,\sigma)$, $F \in P$, $\sigma \in T^{F,i}$.

Given such a good restriction $\rho^{(i+1)}$, 
for every $A^F \in \Gamma_{\lor,i+1}$, we define
$\calT^{(i+1)}(A^F \uhr \rho^{(i+1)})$ to be the height  $t(i+1)+l$ tree
with $T^{F,i}$ (of height $ti$) at the
top, followed by the common trees $T(F,\sigma)$ of height $t$, followed by a bottom
layer of height $l$.
It is not hard to see this tree has the correct form since 
the height $t(i+1)$ subtree (from the root to level $t(i+1)$), which we will call $T^{F,i+1}$, 
consists of $T^{F,i}$ followed by the trees $T(F,\sigma)$, $\sigma \in \Branches(T^{F,i})$,
and therefore is common to all $A^F \in F_{\lor,i+1}$.

Thus we have obtained our desired mapping
$\calT^{(i+1)}$ 
which, for every $F \in P$ and every $A^F \in F_{\lor,i+1}$,
maps $A^F \uhr \rho^{(i+1)}$ to a $(k,H^{(i+1)})$-good decision tree satisfying
the required properties.



\item[(b)] Next consider formulas $A \in \Gamma_{\leq i}$.
Such an $A$ is a subformula of some $F \in P$, so as above we
write this occurrence of $A$ as $A^F$ to indicate that it is a copy of $A$ occurring in $F$.
Since $A^F \in \Gamma_{\leq i}$, 
by the induction hypothesis, the tree
$\calT^{(i)}(A^F \uhr \rho^{(i)})$ is a 
$(ti+1,H^{(i)})$-good decision tree satisfying the additional property that
the top $ti$ layers form a tree $T^{F,i}$ that are common to all $A^F \in F_{\leq i}$.
 
To define $\calT^{(i+1)}(A^F \uhr \rho^{(i+1)})$, we simply extend the tree
$\calT^{(i)}(A^F \uhr \rho^{(i)})$ from the previous phase by replacing
$T^{F,i}$ by $T^{F,i+1}$.
That is, we simply {\it refine} the tree by querying additional
variables. Note that this refinement isn't necesssary, but will
allow the trees for all subformulas $A^F \in F_{\leq i}$ to
have the {\it same} common tree $T^{F,i+1}$ at the top $t(i+1)$ layers,
followed by $l$ layers at the leaves that are specific to $A^F$.


\item[(c)] Next consider formulas $A \in \Gamma_{\neg,i+1}$.
Each such $A$ is a subformula of some $F \in P$, so we will write this
occurrence of $A$ as $A^F$ to indicate that it is a copy of $A$ occurring in $F$.
Since $A^F \in \Gamma_{\neg,i+1}$, it has the form $\neg B^F$ where
$B^F \in F_{i}$ is a subformula of $F$ of depth $i$.
By the induction hypothesis, the tree
$\calT^{(i)}(B^F \uhr \rho^{(i)})$ is a
$(ti+l,H^{(i)})$-good decision tree satisfying properties (1)-(3) of Definition~\ref{def:keval}.
In particular, $\calT^{(i)}(B^F \uhr \rho^{(i)})$ consists of
the common tree $T^{F,i}$ of height $ti$ at the top,
and for each branch $\sigma \in \Branches(T^{F,i})$, the leaf associated with $\sigma$ in $T^{F,i}$ is
labelled with a height-$l$ subtree, $\calT^{(i)}(A_j^F \uhr \rho^{(i)}) \uhr \sigma_j$ (specific to $A_j^F$).
We define $\calT^{(i+1)}(\neg B^F \uhr \rho^{(i+1)}$ to be the tree
$\calT^{(i+1)}(B^F \uhr \rho^{(i+1)})$ (as defined in case (b) since $B^F \in F_{\leq i}$)
but with the leaf values toggled.
It is not hard to see that it is $(k,H^{(i+1)})$-good.

\end{itemize}







It remains to argue that this map $\calT^{(i+1)}(\cdot)$ as defined above satisfies properties (1)-(4) of Definition~\ref{def:keval}.  
Property (1) is immediate.  
For property (2), if $A^F \in F_{\lor,i+1}$, it follows from (a) and (c).
Next we consider  $A \in \Gamma_{\leq i}$. Let $A = \vee_j A_j$, and $\alpha'' \in \Z_2^{V(H^{(i)})}$ denote $\alpha \uhr \rho^{(i)}$ restricted to $V(H^{(i)})$.  By the induction hypothesis, we have that $\calT^{(i)}(A \uhr \rho^{(i)})$ $(H^{(i)}, \alpha'')$-represents $\lor_j \calT^{(i)}(A_j \uhr \rho^{(i)})$.  By two applications of 
(c), it suffices to prove that
\[ \text{$\Prune_{H^{(i+1)},\alpha'}(\calT^{(i)}(A \uhr \rho^{(i)}) \uhr \rho^{(i+1)})$ $(H^{(i+1)}, \alpha')$-represents $\lor_j \Prune_{H^{(i+1)},\alpha'}(\calT^{(i)}(A_j \uhr \rho^{(i)}) \uhr \rho^{(i+1)})$}, \]
which follows from the following lemma (recall that $\alpha' = \alpha'' \uhr \rho^{(i+1)}$ restricted to $V(H^{(i+1)})$): 
\medskip

\begin{lemma}
\label{lemma:prune-preserves-representation-under-or}
Let $k = (\log n)/200d$ and $T_1,\dots,T_\ell$ be $(k,H^{(i)})$-good decision trees over $E(H^{(i)})$, and
let $T$ be a $(k,H^{(i)})$-good decision tree that $(H^{(i)},\alpha'')$-represents
$\lor_j T_j$.  Then $\Prune_{H^{(i+1)}, \alpha'' \uhr \rho^{(i+1)}}(T \uhr \rho^{(i+1)})$ $(H^{(i+1)},\alpha''\uhr \rho^{(i+1)})$-represents
$\lor_j \Prune_{H^{(i+1)}, \alpha''\uhr \rho^{(i+1)}}(T_j \uhr \rho^{(i+1)})$.
\end{lemma}


For property (3), we would like to show that $\calT^{(i+1)}(\neg A \uhr \rho^{(i+1)}) = \calT^{(i+1)}(A \uhr \rho^{(i+1)})^c$ for all
$\neg A \in \Gamma_{i+1}$.
If $\neg A \in \Gamma_{i+1}$ we have:
\begin{align*}
\calT^{(i+1)}(\neg A \uhr \rho^{(i+1)})
&= \Prune_{H^{(i+1)},\alpha'}(\calT^{(i)}(\neg A \uhr \rho^{(i)}) \uhr \rho^{(i+1)})\\
&= \Prune_{H^{(i+1)},\alpha'}(\calT^{(i)}(A \uhr \rho^{(i)})^c \uhr \rho^{(i+1)})\\
&= \Prune_{H^{(i+1)},\alpha'}(\calT^{(i)}((A \uhr \rho^{(i)}) \uhr \rho^{(i+1)})^c)\\
&= \Prune_{H^{(i+1)},\alpha'}(\calT^{(i)}(A \uhr \rho^{(i)}) \uhr \rho^{(i+1)})^c\\
&= \calT^{(i+1)}(A \uhr \rho^{(i+1)})^c,
\end{align*}
where the first equality is by the definition of $\calT^{(i+1)}$ (specifically, (b) if $\neg A \in \Xi_{i+1}$, and (c) if $\neg A \in \Gamma_i$);
the second equality holds because property (2) holds for $\calT^{(i)}$ by the induction hypothesis;
the third equality holds because applying a restriction and toggling the leaf bits
are commutative;
the fourth equality holds because pruning and toggling the leaf bits are commutative; and the last equality holds by the definition of $\calT^{(i+1)}$.

\medskip

For property (4), 
Let $A^l$, $A^r$ be two occurrences of the same formula, $A$, of depth $i+1$.
There are two cases: either $A = \neg B$, or $A = A_1 \lor \ldots A_q$.
where the depth of each $A_i$ is at most $i$.
In the first case, let $A^l = \neg B^l$ and let $A^r = \neg B^r$.
Since $B^l$ and $B^r$ are two occurrences of the same formula of depth $i$,
by the inductive hypothesis $\calT(B^l)$ and $\calT(B^r)$ are consistent
and therefore $\calT(\neg B^l)$ and $\calT(\neg B^r)$ are consistent.
In the second case, let
$A^l = A_1^l \lor \ldots A_q^l$ and let $A^r = A_1^r \lor \ldots A_q^r$,
where each subformula $A_j$ has depth at most $i$.
Consider any pair of consistent paths, $\pi^l$ and $\pi^r$ where $\pi^l$ is a path in $\calT(A^l)$,
and $\pi^r$ is a path in $\calT(A^r)$. We want to show that the leaf values associated with $\pi^r$ and $\pi^l$ are the same.
Assume for sake of contradiction that they are different, and suppose without loss of generality
that $\pi^l$ is a 1-path of
$\calT(A^l)$ and $\pi^r$ is a 0-path of $\calT(A^r)$.
By property (2), $\calT(A^l)$ is consistent with
$\calT(A_1^l),\ldots,\calT(A_q^l)$ and
therefore, there exists some $j \in [q]$ such that $\calT(A_j^l) \uhr \pi^l = 1$.
Now since $A_j^l$ and $A_j^r$ are two occurrences of the same formula of depth $i$,
by induction this implies (by property (4)) that $\calT(A_j^r) \uhr \pi^l =1$.
Now applying property (2) of Definition \ref{def:keval} to $A^r$, since it
represents $\calT(A_1^r),\ldots, \calT(A_q^r)$, this implies that $\calT(A^r) \uhr \pi^l =1$.
Since $\pi^l$ and $\pi^r$ are consistent this implies that $\calT(A^r) \uhr \pi^r =1$, which
contradicts our assumption that $\pi^r$ is a 0-path of $\calT(A^r).


\medskip





Given Lemma~\ref{lemma:prune-preserves-representation-under-or} (the proof of which we defer to the next subsection), we have shown that properties (1)--(4) hold for all $i \in \{0,1,\ldots,d\}$. 

\paragraph{Properties (5) and (6).}  It remains to argue that for each formula $A \in \Gamma_d \uhr \rho^{(d)}$, the tree $\calT^{(d)}(A)$ satisfies properties (5) and (6) of Definition~\ref{def:keval}. 

For property (5), consider a clause $A$ of $\Tseitin(H^{(d)}[\alpha \uhr \rho^{(d)}])$.  Such a clause is one of the four length-3 clauses whose AND gives a constraint from some vertex $v \in V(\exG_n)$; let this vertex be $v$ and let the clause $A$ be $e_1 \vee e_2 \vee e_3$, and let the charge at $v$ be $\alpha(v)=1$.  (Other possibilities can be handled similarly.)  From the base case we have that for each $j \in [3]$, ${\cal T}^{(0)}(e_j \uhr \rho^{(0)})$ is the depth-1 tree $(e_j;0,1)$, and from the $i=0$ case of (a) we have that  $\calT^{(1)}(A \uhr \rho^{(1)})$ is a $(k,H^{(1)})$-good decision tree that 
$(H^{(1)},\alpha\uhr\rho^{(1)})$-represents 
$\vee_{j=1}^3 \Prune_{H^{(1)},\alpha\uhr\rho^{(1)}}( (e_j;0,1) \uhr \rho^{(1)}). $  We will claim that already ${\cal T}^{(1)}(A \uhr \rho^{(1)})$ is a 1-tree, from which property (5) follows.  Seeking a contradiction, suppose there exists $\pi \in \Branches_0(T^{(1)}(A\uhr \rho^{(1)}))$. 
By Definition \ref{def:consistency}, for all three values $j \in [3]$ we have that 
\begin{equation}
\Prune_{H^{(1)},\alpha \uhr \rho^{(1)}}( (e_j;0,1) \uhr \rho^{(1)}) \uhr \closure_{H^{(1)},\alpha \uhr \rho^{(1)}}(\pi) = 0 \quad \text{for $j = 1,2,3$.}
\label{eq:whatever} 
\end{equation} 
Since $\calT^{(1)}(A \uhr \rho^{(1)})$ is $(k,H^{(1)})$-good, we have that $\closure_{H^{(1)},\alpha\uhr\rho^{(1)}}(\pi)$ pushes the contradiction of $\alpha\uhr \rho^{(1)}$ into the giant component of $H-\closure_{H^{(1)}}(\pi)$ (Fact~\ref{fact:Z2-branches-are-good} and Proposition~\ref{prop:closure-is-unique}); this implies that $\rho\circ \closure_{H^{(1)},\alpha\uhr \rho^{(1)}}(\pi)$ is $\alpha$-consistent. However, by Lemma~\ref{lemma:prune-closure-synchs-up} applied to Equation (\ref{eq:whatever}) (noting that the closure of a closed set is itself) we have that 
\[ ((e_j;0,1) \uhr \rho^{(1)}) \uhr \closure_{H^{(1)},\alpha \uhr \rho^{(1)}}(\pi) = 0 \quad \text{for $j=1,2,3$}. \] 
This implies that $(\rho^{(1)} \circ  \closure_{H^{(1)},\alpha \uhr \rho^{(1)}}(\pi))(e_j) = 0$ for $j=1,2,3$, which contradicts the fact that $\rho^{(1)} \circ \closure_{H^{(1)},\alpha \uhr \rho^{(1)}}(\pi)$ is $\alpha$-consistent (since $\alpha(v) = 1$).

It remains to prove property (6) which follows from the following proposition: 

\begin{proposition} 
Fix $(\rho^{(i)},H^{(i)}_n) \in \supp(\calA^{(i)}_n)$ and let $\alpha' =\alpha \uhr \rho^{(i)}$.  Let $T_0,T_1,\ldots,T_6$ be $(k,H^{(i)}_n)$-good decision trees where \red{$k = (\log n)/200d$}. Then for every $\pi_0 \in \Branches(T_0)$, there exist $\pi_i \in \Branches(T_i)$ for $i\in [6]$ such that 
\begin{enumerate}
\item $\{ \pi_0,\ldots,\pi_6\}$ is mutually compatible.
\item $\pi^\ast := \closure_{H^{(i)},\alpha'}(\pi_0 \circ \cdots \circ \pi_6)$ pushes the contradiction of $\alpha'$ into the giant component of $H - \supp(\pi^\ast)$.
\end{enumerate} 

\end{proposition} 


\begin{proof} 
Since $\pi_0$ is $H^{(i)}$-independent, we have that $\pi_0$ pushes the contradiction of $\alpha'$ into the giant component of $H^{(i)} - \supp(\pi)$. Equivalently, the $(\alpha' \uhr \pi_0)$-charge of a component $C$ of $H^{(i)} - \supp(\pi_0)$ is odd iff $C$ is giant (note that $H^{(i)}-\supp(\pi_0)$ is connected). 


Consider $T_1 \uhr \pi_0$, a decision tree over $E(H^{(i)} - \supp(\pi_0))$. Observe that $$\Branches_\bot(\Prune_{H^{(i)}-\supp(\pi_0),\alpha' \uhr \pi_0}(T_1 \uhr \pi_0)) = \emptyset$$  by Lemma~\ref{lemma:prune-closure-synchs-up-bottom} since $(H^{(i)} - \supp(\pi_0)) - \closure_{H^{(i)}-\supp(\pi_0)}(\tilde{\pi}_1)$ has a giant component (by Fact~\ref{fact:break-off-small-in-H} using $|H^{(i)}| \ge \sqrt{n}$ and $k = (\log n)/200d$). Therefore, we may fix $$\tilde{\pi} \in  \Branches_b(\Prune_{H^{(i)}-\supp(\pi_0),\alpha' \uhr \pi_0}(T_1 \uhr \pi_0))$$ for some $b\in \Z_2$, and by Fact~\ref{fact:Z2-branches-are-good}, we have that $\tilde{\pi}_1$ pushes the contradiction of $\alpha' \uhr \pi_0$ into the giant component of $(H^{(i)} - \supp(\pi_0)) - \supp(\tilde{\pi}_1)$.  By Proposition~\ref{prop:closure-is-unique}, we have that $\closure_{H^{(i)}-\supp(\pi_0),\alpha'\uhr \pi_0}(\tilde{\pi}_1)$ pushes the contradiction of $\alpha' \uhr \pi_0$ into the giant component of $(H^{(i)} - \supp(\pi_0)) - \closure_{H^{(i)}-\supp(\pi_0)}(\tilde{\pi}_1)$. Equivalently, 
\begin{itemize}
\item[($\dagger$)] $\pi_0 \circ \closure_{H^{(i)}-\supp(\pi_0),\alpha'\uhr \pi_0}(\tilde{\pi}_1)$ pushes the contradiction of $\alpha'$ into the giant component of $H^{(i)} - \supp(\pi_0) - \closure_{H^{(i)}-\supp(\pi_0)}(\tilde{\pi}_1)$.  
\end{itemize} 
Recall that $\tilde{\pi}_1 \in \Branches_b(\Prune_{H^{(i)}-\supp(\pi_0),\alpha' \uhr \pi_0}(T_1 \uhr \pi_0))$. By Lemma~\ref{lemma:prune-closure-synchs-up}, we have that 
\[ (T_1 \uhr \pi_0) \uhr \closure_{H^{(i)} - \supp(\pi_0),\alpha' \uhr \pi_0}(\tilde{\pi}_1) = b. \] 
This implies the existence of a path $\pi_1 \in \Branches_b(T_1)$ such that $\pi_1$ is a subrestriction of $\pi_0 \circ \closure_{H^{(i)} - \supp(\pi_0),\alpha' \uhr \pi_0}(\tilde{\pi}_1)$. Note that $\pi_1$ is consistent with $\pi_0$, and since $\pi_0 \circ \pi_1$ is a subrestriction of $\pi_0 \circ \closure_{H^{(i)} - \supp(\pi_0),\alpha' \uhr \pi_0}(\tilde{\pi}_1)$ it follows from ($\dagger$) that $\pi_0 \circ \pi_1$ pushes the contradiction of $\alpha'$ into the giant component of $H^{(i)} - \supp(\pi_0 \circ \pi_1)$.  

The existence of $\pi_2,\dots,\pi_6$ with the claimed properties follows by repeating the above argument, where to get the argument started we observe that (as we have just shown) $\pi_0 \circ \pi_1$ pushes the contradiction of $\alpha'$ into the giant component of $H^{(i)}- \supp(\pi_0 \circ \pi_1)$. Since $|\pi_0 \cup \cdots \cup \pi_6| \le 7k = 7(\log n)/200d$, we apply Fact~\ref{fact:break-off-small-in-H} and Proposition~\ref{prop:closure-is-unique} to conclude that $\pi^\star := \closure_{H^{(i)},\alpha'}(\pi_0 \circ \cdots \circ \pi_6)$ pushes the contradiction of $\alpha'$ into the giant component of $H^{(i)}- \supp(\pi^\star)$. 
\end{proof} 

This concludes the proof of Lemma~\ref{lemma:restriction-evaluation}, modulo the proof of Lemma~\ref{lemma:prune-preserves-representation-under-or}. 

\end{proof}

\subsection{Proof of Lemma~\ref{lemma:prune-preserves-representation-under-or}}

We will need the following lemma: 

\begin{lemma}
\label{lemma:bacon-saver-stringy} 
Fix $(\rho^{(i)}, H^{(i)})\in \supp(\calA^{(i)})$ and $(\rho^{(i+1)},H^{(i+1)}) \in \supp(\calA^{(i+1)}(\rho^{(i)},H^{(i)}))$, and let $\alpha'' = \alpha \uhr \rho^{(i)}$. Let $\pi$ be a restriction to the edges in $E(H^{(i+1)})$ such that $\supp(\pi)$ is an $H^{(i+1)}$-independent set of size at most $\red{\tau(i+1,n)/3\lambda^\star}$, where $\lambda^\star$ is the $\lambda^\star$ from from Fact~\ref{fact:break-off-small-in-H}.  Let $\beta$ be a sub-restriction of $\rho \circ \closure_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(\pi)$ where $\supp(\beta)$ is a $H^{(i)}$-independent set of size at most $\red{\tau(i+1,n)/3\lambda^\star}$.  Then $\rho\circ \closure_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(\pi)$ extends $\closure_{H^{(i)},\alpha''}(\beta)$.
\end{lemma} 

\begin{proof} 
For notational clarity we prove the $i=0$ case, noting that the proof of the general case proceeds along essentially identical lines. In this case  $\rho^{(0)} = \{ \ast\}^{E(\exG_n)}$, $H^{(0)} = \exG_n$, and $\alpha'' = \alpha$. We write $n'$ for $\tau(1,n)$, the number of real vertices of $H^{(1)}$. 

Note that $\rho^{(1)} \circ \closure_{H^{(1)},\alpha \uhr\rho^{(1)}}(\pi)$ extends $\beta$, and so the lemma statement is equivalent to the claim that every edge $e\in (\closure_{\exG_{n}}(\supp(\beta)) \setminus \supp(\beta))$ is fixed to the same constant $b\in \Z_2$ by $\closure_{\exG_{n},\alpha}(\beta)$ and by $\rho^{(1)} \circ \closure_{H^{(1)},\alpha\uhr \rho^{(1)}}(\pi)$.  Fix any such edge $e$, and recall that $e$ is a bridge in $\exG_{n} - \supp(\beta)$.  Since $\exG_{n} - \supp(\rho^{(1)} \circ \closure_{H^{(1)},\alpha\uhr\rho^{(1)}}(\pi)) = H^{(1)} - \closure_{H^{(1)}}(\supp(\pi))$ is bridgeless and $\rho^{(1)}\circ \closure_{H^{(1)},\alpha\uhr \rho^{(1)}}(\pi)$ extends $\beta$, it follows that $e$ is also fixed by $\rho^{(1)}\circ \closure_{H^{(1)},\alpha \uhr \rho^{(1)}}(\pi)$; it remains to argue that $\closure_{\exG_{n},\alpha}(\beta)$ and $\rho^{(1)} \circ \closure_{H^{(1)/}\alpha \uhr\rho^{(1)}}(\pi)$ fix $e$ to the  same constant. 


Since $|\supp(\pi)| \le n'/3\lambda^\star$, it follows from Fact~\ref{fact:break-off-small-in-H} that $H^{(1)} - \closure_{H^{(1)}}(\supp(\pi))$ has a giant component. We may then apply Proposition~\ref{prop:closure-is-unique} (recall that $\supp(\pi)$ is $H^{(1)}$-independent) to get that 
\begin{itemize}
\item[($\dagger$)] $\closure_{H^{(1)},\alpha \uhr \rho^{(1)}}(\pi)$ pushes the contradiction of $\alpha\uhr \rho^{(1)}$ into the giant component of $H^{(1)}-\closure_{H^{(1)}}(\supp(\pi))$ (of size $> |V(H^{(1)})|/2$).
\end{itemize} 
Since $\supp(\beta)$ is $\exG_{n}$-independent, we have that $\exG_{n}-\supp(\beta)$ is connected and has $e$ as bridge. Let $C_1$ and $C_2$ be the two components of $\exG_{n}-(\supp(\beta) \cup\{e\})$ where $|V(C_1)| \ge |V(C_2)|$ and $|V(C_1)| + |V(C_2)| = |V(\exG_{n})|= n$. Since $|\supp(\beta)| \le n'/3\lambda^\star$, it follows from Fact~\ref{fact:break-off-small-in-H} that $|V(C_2)| \le n'/3 < |V(H^{(1)})|/3$ and $|V(C_1)| \ge n-n'/3 > n/2$. 
Recall that the $(\alpha\uhr \beta)$-charge of $\exG_{n}-\supp(\beta)$ is odd since $\supp(\beta)$ is $\exG_{n}$-independent. Therefore $\closure_{G,\alpha}(\beta)$ fixes $e$ according to the unique assignment $b\in \Z_2$ so that the induced $(\alpha \uhr \beta \circ e \to b)$-charge of $C_1$ is odd and that of $C_2$ is even. We claim that $\rho^{(1)}\circ \closure_{H^{(1)},\alpha\uhr \rho^{(1)}}(\pi)$ fixes $e$ to the same value $b$. If not, $\rho^{(1)} \circ \closure_{H^{(1)},\alpha \uhr \rho^{(1)}}(\pi)$ extends $(\beta\circ e \to \bar{b})$ where $(\beta \circ e \to \bar{b})$ does \emph{not} push the contradiction of $\alpha$ into the giant component of $\exG_n - (\supp(\beta)\cup \{ e\})$; by Fact~\ref{fact:push-sub-super} this contradicts ($\dagger$).This completes the proof of Lemma~\ref{lemma:bacon-saver-stringy}.
\end{proof} 



We are now ready to prove Lemma~\ref{lemma:prune-preserves-representation-under-or}: 

\begin{proof}[Proof of Lemma~\ref{lemma:prune-preserves-representation-under-or}]
Let $T^* := \Prune_{H^{(i+1)}, \alpha'' \uhr \rho^{(i+1)}}(T \uhr \rho^{(i+1)})$. We first recall that ``$T^* (H^{(i+1)},\alpha''\uhr \rho^{(i+1)})$-represents   
$\lor_j \Prune_{H^{(i+1)}, \alpha''\uhr \rho^{(i+1)}}(T_j \uhr \rho^{(i+1)})$'' means:
\[ \pi \in \Branches_b(T^*) \Longrightarrow (\lor_j\,\Disj(\Prune_{H^{(i+1)},\alpha''\uhr\rho^{(i+1)}}(T_j \uhr \rho^{(i+1)}))) \uhr  \closure_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(\pi) = b. \]

We consider two cases depending on whether $b = 1$ or $0$. If $b=1$, it suffices to argue that 
\[ \pi \in \Branches_1(T^*) \Longrightarrow \exists\,j \colon \Prune_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(T_j \uhr \rho^{(i+1)}) \uhr  \closure_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(\pi) = 1. \] 
 
Fix $\pi \in \Branches_1(T^*)$. Since $T^*$ has height at most $\red{k = (\log n)/200d}$ it follows from Fact~\ref{fact:break-off-small-in-H} that $H^{(i+1)} -  \closure_{H^{(i+1)}}(\supp(\pi))$ has a giant component. Hence we can apply Lemma~\ref{lemma:prune-closure-synchs-up} and get that 
\[ (T \uhr \rho^{(i+1)}) \uhr \closure_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(\pi) = 1. \] 
This implies that there exists $\pi' \in \Branches_1(T)$ such that $\pi'$ is a sub-restriction of $\rho^{(i+1)} \circ \closure_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(\pi)$. 

Recall our assumption that $T$ $(H^{(i)},\alpha'')$-represents $\lor_j T_j$. This means that 
\begin{align*}
\pi' \in \Branches_1(T) &\Longrightarrow \ \exists\,j \colon T_j \uhr \closure_{H^{(i)},\alpha''}(\pi') = 1. 
\end{align*} 
Fix such an index  $j$. By Lemma~\ref{lemma:bacon-saver-stringy}, we have that $\closure_{H^{(i)},\alpha''}(\pi')$ is a sub-restriction of $\rho^{(i+1)} \circ \closure_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(\pi)$, and so we have that 
\[ (T_j \uhr \rho^{(i+1)}) \uhr \closure_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(\pi) = 1.\] 

Observe that $T_j \uhr \rho^{(i+1)}$ is total and has depth at most $k$. It follows from Lemma~\ref{lemma:prune-closure-synchs-up-bottom}, Fact~\ref{fact:break-off-small}, and inspection of the $\Prune$ procedure that $\Prune_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(T_j \uhr \rho^{(i+1)})$ is total as well. Hence we may apply Fact~\ref{fact:prune-self-evident} to obtain that


\[ \Prune_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(T_j \uhr \rho^{(i+1)}) \uhr  \closure_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(\pi) = 1, \] 
which completes the proof of the $b=1$ case.


For the $b=0$ case, fix $\pi \in \Branches_0(T^*)$. In this case it suffices to argue that for all $j$, either 
\begin{equation} \Prune_{H^{(i+1)},\alpha''\uhr\rho^{(i+1)}}(T_j \uhr \rho^{(i+1)}) \uhr  \closure_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(\pi) = 0 \label{eq:case1}
\end{equation} 
or  
\begin{equation} \Prune_{H^{(i+1)},\alpha''\uhr\rho^{(i+1)}}(T_j \uhr \rho^{(i+1)}) \uhr  \closure_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(\pi) \text{ is a $0$-tree}. \label{eq:case2}
\end{equation} 
Since $T^*$ has height at most $\red{k = (\log n)/200d}$ it follows from Fact~\ref{fact:break-off-small-in-H} that $H^{(i+1)} -  \closure_{H^{(i+1)}}(\supp(\pi))$ has a giant component. Hence we can apply Lemma~\ref{lemma:prune-closure-synchs-up} and get that 
\[ (T \uhr \rho^{(i+1)}) \uhr \closure_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(\pi) = 0. \] 
This implies that there exists $\pi' \in \Branches_0(T)$ such that $\pi'$ is a sub-restriction of $\rho^{(i+1)} \circ \closure_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(\pi)$. 

Recall our assumption that $T$ $(H^{(i)},\alpha'')$-represents $\lor_j T_j$. This means that 
\begin{align*}
\pi' \in \Branches_0(T) &\Longrightarrow \ \forall\,j \colon \text{ either } T_j \uhr \closure_{H^{(i)},\alpha''}(\pi') = 0, \text{or } T_j \uhr \closure_{H^{(i)},\alpha''}(\pi') \text{ is a $0$-tree.}   
\end{align*} 
By Lemma~\ref{lemma:bacon-saver-stringy}, we have that $\closure_{H^{(i)},\alpha''}(\pi')$ is a sub-restriction of $\rho^{(i+1)} \circ \closure_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(\pi)$, and so we have that for all $j$, either
\[ (T_j \uhr \rho^{(i+1)}) \uhr \closure_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(\pi) = 0 \text{ or } (T_j \uhr \rho^{(i+1)}) \uhr \closure_{H^{(i+1)},\alpha''\uhr \rho^{(i+1)}}(\pi) \text{ is a $0$-tree.}\] 
Again by Fact~\ref{fact:prune-self-evident}, it follows that either (\ref{eq:case1}) or (\ref{eq:case2}) holds, and the proof is complete. 
}
\end{proof}






==> otherdefs.tex <==

\subsection{Restrictions and Decision Trees}

Given a set of variables $E$, a \emph{restriction $\beta$} is an element of $(\Z_2 \cup \{\ast\})^E$.  We may equivalently view $\beta$ as an element of $\Z_2^{S}$ for some $S \subseteq E$, and we say that $S$ is the \emph{support of $\beta$}, denoted $\supp(\beta).$   Given restrictions $\beta,\beta' \in (\Z_2 \cup \{\ast\})^E$ we say that $\beta'$ is a \emph{sub-restriction} of $\beta$ if $\supp(\beta') \subseteq \supp(\beta)$ and $\beta(e) =b \in \Z_2$ whenever $\beta'(e)=b \in \Z_2.$  We say that $\beta$ is an \emph{extension} of $\beta'$ if $\beta'$ is a sub-restriction of $\beta.$   We say that a set of restrictions $\{\beta_1,\dots,\beta_t\}$ is \emph{mutually compatible} if for every $i,j \in [t]$ we have that $\beta_i(e)=\beta_j(e)$ whenever $e \in \supp(\beta_i) \cap \supp(\beta_j)$.

A decision tree is said to be \emph{proper} if no variable is queried two or more times on any branch.  Throughout the entire paper all decision trees are assumed to be proper unless explicitly stated otherwise.

Let $T$ be a decision tree over a space of variables $E$ and let $\beta$ be a restriction.  We write ``$T \uhr \beta$'' to denote the decision tree obtained by simplifying $T$ according to $\beta$  ``in the obvious way.''  More precisely, if $T=(e;T_0,T_1)$, meaning that $T$ is the decision tree with variable $e$ at the root and left (respectively, right) child $T_0$ (respectively, $T_1$), then we have the following:

\begin{itemize}

\item If $\beta(e)=\ast$ then $T \uhr \beta = (e; T_0 \uhr \beta; T_1 \uhr \beta)$;

\item If $\beta(e)=0$ then $T \uhr \beta = T_0 \uhr \beta$;

\item If $\beta(e)=1$ then $T \uhr \beta = T_1 \uhr \beta$.

\end{itemize}

For $b \in \Z_2$, we write ``$T \uhr \beta = b$'' to indicate that $T \uhr \beta$ is the $1$-node tree consisting only of a leaf $b$.

A \emph{branch} of a decision tree $T$ over variable set $E$ is a root-to-leaf path (which, more formally, is a sequence $\pi = \pi_1 \circ \dots \circ \pi_k$ where each $\pi_i$ is an element of $E \times \Z_2$ and no element occurs twice in $\pi$).  Clearly every branch in a decision tree $T$ corresponds to a unique restriction and we will often take this perspective of viewing branches as restrictions.  

Unless specified otherwise a decision tree is assumed to have every leaf labeled with an element of $\Z_2$; we sometimes refer to such trees as \emph{total} to emphasize that every leaf is labeled with an element of $\Z_2.$   A \emph{partial decision tree} is a decision tree in which each leaf is labeled with some element of $\Z_2 \cup \{\bot\}$.   A partial decision tree is said to be \emph{$m$-safe} if all leaves labeled $\bot$ are at depth $\geq m.$  Given a total decision tree $T$, we write $T^c$ to denote the tree obtained from $T$ by replacing each leaf bit with its complement.

For $b \in (\Z_2 \cup \{\bot\})$ and a decision tree $T$ let $\mathrm{Branches}_b(T)$ denote the set of branches of $T$ whose leaf is labeled $b$. Let $\mathrm{Branches}(T) = \mathrm{Branches}_0(T) \cup \mathrm{Branches}_1(T)$, which is the set of all branches of $T$ if $T$ is total. Note that if $T\uhr \beta = b$ for some $b \in \Z_2$ (i.e.~$T \uhr \beta$ is the constant-$b$ tree of depth $0$), then there exists a path $\pi \in \Branches_b(T)$ such that $\beta$ extends $\pi$.

A $1$-tree is a decision tree in which every leaf is labeled by $1$, and likewise $0$-tree.

We close this subsection with a notational convention:  many of our definitions, lemmas, etc. will involve restrictions.  As a helpful notational convention, in such definitions, lemmas, etc. we use $\rho,\rho',\tilde{\rho},$ etc.\ to denote restrictions which should be thought of as ``coming from'' a random restriction process, and we use $\pi, \pi', \tilde{\pi},$ etc. to denote restrictions which should be thought of as ``coming from'' a branch in some decision tree.  If the definition/lemma/etc.\ may arise in either context we use $\beta,\beta',\tilde{\beta},$ etc.



\subsection{DNFs and Formulas} \label{sec:DNFs-formulas}


Observe that any element of $\Branches_1(T)$, for any decision tree $T$, corresponds to a conjunction in an obvious way, so we may view $\Branches_1(T)$ as a collection of conjunctions (i.e.\ of terms).
Given a decision tree $T$ we write ``$\Disj(T)$'' to denote the
DNF whose terms correspond precisely to the 1-branches of $T$.
Observe that if $T_1,\dots$ are decision trees then
``$\lor_j \Disj(T_j)$'' is a DNF (whose terms are precisely the terms
that occur in some $\Disj(T_j)$).




For a term $t$, and a restriction $\beta$, $t \uhr {\beta}$ is 0 if any literal in $t$ is set to $0$
by $\beta$, otherwise, $t \uhr {\beta}$ is the conjunction of literals
that are unset by $\beta$. (By definition, a term of size zero is equal to 1.)
For an DNF formula $F = t_1 \lor \ldots \lor t_m$,
$F \uhr {\beta}$ is the DNF formula obtained as follows:
If any term is set to $1$ by $\beta$, then $F \uhr {\beta} =1$, and otherwise
$F_{\beta} = \lor_i  (t_i \uhr {\beta})$. 
In particular, $F \uhr \beta=0$ means that every term in $F$ is
set to 0 by $\beta.$



For a Boolean formula $A$ and a restriction $\beta$,  $A \uhr \beta$ denotes the formula obtained by performing simple variable substitution as dictated by $\beta$.  If $\Gamma$ is a collection of formulas $\Gamma = \{A_i\}$ then $\Gamma \uhr \beta$ denotes $\{A_i \uhr \beta\}.$



\subsection{Tseitin contradictions} \label{sec:tseitin}

Given a labeling $ \alpha \in  \Z_2^{V}$
of the vertices of a graph $G=(V,E)$, we define a Boolean formula associated with $(G,\alpha)$.   We view each element of $E$ as a formal Boolean variable.  The Tseitin formula $\Tseitin(G[\alpha])$ over the formal variables in $E$ is defined to be 
\[ \Tseitin(G[\alpha]) := \bigwedge_{v\in V} \underbrace{\Big( \sum_{e \sim v} e = \alpha(v)\Big)}_{\text{constraint}(v,\alpha)},\]
where ``$e \sim v$'' indicates that edge $e$ has vertex $v$ as an endpoint.
Note that if $G$ has maximum degree 3, then for every $v\in V$, $\text{constraint}(v,\alpha)$ can be expressed as a $3$-CNF with $2^{3-1} = 4$ clauses. Therefore for such an $n$-node graph, the formula $\Tseitin(G[\alpha])$ is a $3$-CNF with $4n$ clauses. 

We sometimes refer to $\alpha$ as the ``charge'' of $G$, and to the value $\alpha(v)$ as being ``odd'' or ``even.'' 
The following fact is well known (see e.g.~Lemma 18.16 of \cite{Jukna:12}):

\begin{fact} \label{fact:basic-tseitin}
If $G$ is connected, then
$\Tseitin(G[\alpha])$ is satisfiable iff $\sum_{v\in V} \alpha(v) = 0$.  
\end{fact} 

For $G$ a  graph and $\alpha$ a charge we say that $\alpha$ is an \emph{odd charge} if $\sum_{v \in V} \alpha(v)=1$ and that it is an \emph{even charge} otherwise.  By Fact \ref{fact:basic-tseitin}, if $ \alpha \in  \Z_2^{V}$ is any odd charge then the associated 3-CNF is unsatisfiable.  We sometimes also consider charges $\alpha \in \Z_2^{V'}$ for some $V' \sse V$, as in the following definition and facts.  (Here and throughout the paper, for a graph $G = (V,E)$ and $S \subseteq E$, we write $G-S$ to denote the graph $(V,E\setminus S)$.) 
 

\begin{definition}[$\alpha$-consistency]
Let $G = (V,E)$ be a graph and $\alpha \in \Z_2^{V'}$ where $V' \sse V$. Let $S \sse E$ be a subset of the edges and $\rho \in \Z_2^S$. We say that $\rho$ is \emph{$\alpha$-consistent} if 
\[ \sum_{e \sim v} \rho(e) = \alpha(v) \quad \text{for all $v \in V'$ that are isolated in $G- S$.}\] 
\end{definition}


The following fact is an easy consequence of Fact \ref{fact:basic-tseitin}:

\begin{fact}
\label{fact:tseitin-satisfiable} 
Let $G = (V,E)$ be a connected graph and $\alpha \in \Z_2^{V'}$ where $V' \subsetneq V$. Then there is an $\alpha$-consistent assignment $\rho \in \Z_2^{E(G)}$. 
\end{fact}  
\begin{proof} If the charge $\alpha$ is even then this follows from Fact \ref{fact:basic-tseitin}.  If the charge $\alpha$ is odd then ...
\end{proof}

\begin{fact}
\label{fact:tseitin-subspace} 
Let $G = (V,E)$ be a connected graph and $\alpha \in \Z_2^{V'}$ where $V' \subsetneq V$. Then the set of all $\alpha$-consistent assignments $\rho \in \Z_2^{E(G)}$ forms an affine subspace of $\Z_2^{E(G)}$.  
\end{fact} 


\begin{proof}
The set of $\alpha$-consistent assignments is easily seen to be the set of solutions to a system of linear equations; this system is satisfiable (by Fact~\ref{fact:tseitin-satisfiable}), and therefore the set of solutions forms an affine subspace.
\end{proof} 


\begin{definition}[Restricting a charge] 
Let $G = (V,E)$ be a graph and $\alpha \in \Z_2^V$. Let $S \sse E$ be a subset of the edges and $\rho \in \Z_2^S$.  We define $(\alpha \uhr \rho) \in \Z_2^V$ by  
\[ (\alpha \uhr \rho)(v) = \alpha(v) - \sum_{e \sim v} [e\in S\ \&\ \rho(e) = 1] \quad \text{for all vertices $v \in V$}.\] 
\end{definition} 


We say that a connected component $C = (V(C),E(C))$ of an $n$-node graph is \emph{giant} if $V(C) > n/2$. Note that there can only be one giant component in any given graph.  For $\alpha \in \Z_2^{V}$ a charge of $G$ and $C=(V(C),E(C))$ a connected component of $G$, we say the \emph{$\alpha$-charge of $C$} is $\sum_{v \in C} \alpha(v).$  

We mention that sometimes we will write things like $H[\alpha]$ when $\alpha \in \Z_2^{V(G)}$ and $H$ is a subgraph of $G$ where $V(H)$ is a proper subset of $V(G)$; in such a usage ``$\alpha$'' should be interpreted as
$\alpha$ restricted to $V(H).$


